Neural Network Compatible Off-Policy Natural Actor-Critic Algorithm

Learning optimal behavior from existing data is one of the most important problems in Reinforcement Learning (RL). This is known as "off-policy control" in RL where an agent's objective is to compute an optimal policy based on the data obtained from the given policy (known as the behavior policy). As the optimal policy can be very different from the behavior policy, learning optimal behavior is very hard in the "off-policy" setting compared to the "on-policy" setting where new data from the policy updates will be utilized in learning. This work proposes an off-policy natural actor-critic algorithm that utilizes state-action distribution correction for handling the off-policy behavior and the natural policy gradient for sample efficiency. The existing natural gradient-based actor-critic algorithms with convergence guarantees require fixed features for approximating both policy and value functions. This often leads to sub-optimal learning in many RL applications. On the other hand, our proposed algorithm utilizes compatible features that enable one to use arbitrary neural networks to approximate the policy and the value function and guarantee convergence to a locally optimal policy. We illustrate the benefit of the proposed off-policy natural gradient algorithm by comparing it with the vanilla gradient actor-critic algorithm on benchmark RL tasks.

==> convergence-analysis.tex <==
\section{Sketch of Convergence of the algorithm}
In this section, we outline the convergence of our proposed algorithm. As the algorithm uses neural network architecture for policy and value function computations, some assumptions are needed for the convergence of the algorithm, which we state and discuss as we go along. 

We first briefly discuss the two-timescale stochastic approximation scheme \cite{borkar2009stochastic}. Suppose there are two updates of the following form:
\begin{align} \label{conv-1}
    &x_{n+1} = x_n + a(n) [h(x_n,y_n)+ M^1_{n+1}], \\ 
    &y_{n+1} = y_n + b(n) [g(x_n,y_n)+M^2_{n+1}], \label{conv-2}
\end{align}
where $h$ and $g$ are Lipschitz functions and $\{M^1\}$, $\{M^2\}$ are Martingale difference sequences, $\{a(n)\}$ and $\{b(n)\}$ are step-size sequences. 

In the two-timescale stochastic approximation scheme, the update \eqref{conv-1} is carried out at a faster rate compared to \eqref{conv-2}. Let $\lambda(y)$ denote the point where the update \eqref{conv-1} converges to, when constant $y$ is chosen, i.e., $h(x_n,y_n)$ is replaced with $h(x_n,y)$. Now, consider a modified \eqref{conv-2} as follows:
\begin{align}\label{conv-3}
    y_{n+1} = y_n + b(n) [g(\lambda(y_n),y_n)+M^2_{n+1}]
\end{align}
Let the $\{y_n\}$ iterates in \eqref{conv-3} converge to $y^*$.
Then, under conditions defined in \cite[Chapter 6]{borkar2009stochastic}, one can show that, 
\begin{align}
    (x_n,y_n) \xrightarrow{} (\lambda(y^*), y^*).
\end{align}

In our proposed algorithm, the policy updates $\theta$ are performed slowly compared to the advantage value function parameter ($x$) updates. Before, we adapt our algorithm updates as \eqref{conv-1}-\eqref{conv-2}, we make certain assumptions on the value function network. 

\begin{assumption}\label{a1}
The value function network at every iteration $t, ~ t \geq 0$ computes unbiased value function corresponding to policy $\pi_{\theta_t}$. 
\end{assumption}

\begin{assumption}\label{a2}
$\displaystyle \sum_{n= 0}^{\infty} \alpha_n = \sum_{n= 0}^{\infty} \beta_n = \infty, ~ \displaystyle \sum_{n= 0}^{\infty} (\alpha_n + \beta_n)^2 < \infty, ~ \frac{\beta_n}{\alpha_n} \xrightarrow{} 0$.  
\end{assumption}

Let the policy parameters at time $n$ be $\theta_n$. Also, let $s_n \sim \Tilde{d_\mu}(.), a_n \sim \mu(s,.), s'_n \sim P(.|s_n,a_n)$ be the sample obtained at time $n$. Following the Assumptions \ref{a1} and \ref{a2}, the update rule for $x_{n+1}$ (step 9 of the Algorithm \ref{alg:NAC}) can be re-written as follows:
\begin{align}\label{ca-1}
x_{n+1} = x_{t} + \alpha_n \displaystyle (h(x_n,\theta_n) + M^1_{n+1}),
\end{align}
where $h(x_n,\theta_n) = -\frac{1}{2}\nabla_x \displaystyle \E_{s\sim \Tilde{d}_{\pi_{\theta_n}}, a \sim \pi_{\theta_n}}[(A^{\pi_{\theta_n}(s,a)} - x_n^T \nabla_{\theta}\log \pi_{\theta_n}(s,a))^2]$ and $M^1_{t+1} = w_{\theta_n}(s_n) \rho(s_n,a_n)(r_n + \gamma V_{\psi}(s'_n) -V_{\psi}(s_n) - x_n^T\nabla_{\theta}\pi_{\theta_n}(s_n,a_n))\nabla_{\theta}\pi_{\theta_n}(s_n,a_n) - h(x_n,\theta_n)$.
Let $\mathcal{F}_n = \sigma \{\theta_0,x_0,s_k,a_k,s'_k ~ k \leq n\}$ be the increasing family of sigma-fields. Then, we have $\E[M^1_{t+1}\mid \mathcal{F}_n]$
\begin{align*}
    &= \E_{s\sim \Tilde{d}_{\mu}, a \sim \mu}[w_{\theta_n}(s_n) \rho(s_n,a_n)(r_n + \gamma V_{\psi}(s'_n) -V_{\psi}(s_n)- x_n^T\nabla_{\theta}\pi_{\theta_n}(s_n,a_n))\nabla_{\theta}\pi_{\theta_n}(s_n,a_n)] - h(x_n,\theta_n) \\
    &= \E_{s\sim \Tilde{d}_{\pi_{\theta_n}}, a \sim \pi_{\theta_n}}[(A^{\pi_{\theta_n}}(s,a) - x_n^T \nabla_{\theta}\log \pi_{\theta_n}(s,a))\nabla_{\theta}\pi_{\theta_n}(s,a)]  - h(x_n,\theta_n) \\
    &= 0.
\end{align*}

Therefore, $\{M^1_{t}\}$ is a zero mean Martingale sequence. 
Similarly, the update for the policy parameter $\theta$ (step 10 of the Algorithm \ref{alg:NAC})  can be re-written as:
\begin{align}
    \theta_{n+1} = \theta_n + \beta_n g(x_n,\theta_n),
\end{align}
where $g(x_n,\theta_n) = x_n$. 

Let us first analyse \eqref{ca-1}. If a constant $\theta$ is used in the place of $\theta_n$, then $x_n,$ as $n \xrightarrow{} \infty,$ converges to a point $\lambda(\theta),$ such that,
\begin{align}
     \E[(A^{\pi_{\theta}}(s,a) - \lambda(\theta)^T \nabla_{\theta} \log \pi_{\theta}(s,a)) \nabla_{\theta} \log \pi_{\theta}(s,a) ]= 0.
\end{align}

Finally, the iteration given by:
\begin{align}
    \theta_{n+1} = \theta_n + \beta_n g(\lambda(\theta_n),\theta_n),
\end{align}
converges to $\theta^*$, where $\nabla_{\theta}J(\theta)\mid_{\theta = \theta^*} = 0$.

From the theory of two time-scale stochastic approximation discussed above, we can conclude that the policy parameter $\theta_n$ update given in step 10 of Algorithm \ref{alg:NAC}:
\begin{align}
    \theta_n \xrightarrow{} \theta^*,
\end{align}
almost surely.
